CUP: A Conservative Update Policy Algorithm for Safe Reinforcement Learning

Safe reinforcement learning (RL) is still very challenging since it requires the agent to consider both return maximization and safe exploration. In this paper, we propose CUP, a Conservative Update Policy algorithm with a theoretical safety guarantee. We derive the CUP based on the new proposed performance bounds and surrogate functions. Although using bounds as surrogate functions to design safe RL algorithms have appeared in some existing works, we develop them at least three aspects: (i) We provide a rigorous theoretical analysis to extend the surrogate functions to generalized advantage estimator (GAE). GAE significantly reduces variance empirically while maintaining a tolerable level of bias, which is an efficient step for us to design CUP; (ii) The proposed bounds are tighter than existing works, i.e., using the proposed bounds as surrogate functions are better local approximations to the objective and safety constraints. (iii) The proposed CUP provides a non-convex implementation via first-order optimizers, which does not depend on any convex approximation. Finally, extensive experiments show the effectiveness of CUP where the agent satisfies safe constraints. We have opened the source code of CUP at https://github.com/RL-boxes/Safe-RL.

==> abstract.tex <==
%!TEX root = main.tex
We focus on using Thompson Sampling to solve unimodal bandit problems, where the expected reward is monotonic over the partially ordered arms.
Although \cite{paladino2017unimodal,trinh2020solving} have extended Thompson Sampling to unimodal multi-armed bandits, 
their methods heavily depend on a \emph{forced-exploitation} mechanism that forces the player to pull the current leader (i.e., the action maintains the maximal empirical mean of rewards) at a fixed frequency.
Forced-exploitation separates exploration from exploitation rounds, which is undesirable for multi-armed bandit problems.
Additionally,
tuning the frequency factor manually for the forced-exploitation method is inefficient for complex sequence decision-making tasks, 
and it is still a debate that whether or not those forcing mechanisms are desirable for unimodal bandits.



To address the above problems, we propose the $\texttt{FEF}$-$\texttt{UTS}$ (forced-exploitation free unimodal Thompson Sampling) algorithm.
The proposed $\texttt{FEF}$-$\texttt{UTS}$ does not consider the forced-exploitation mechanism, i.e.,
$\texttt{FEF}$-$\texttt{UTS}$ does not force the player to pull the current leader.
To exploit the unimodal structure better, 
at each step, instead of exploration from the entire decision space,
$\texttt{FEF}$-$\texttt{UTS}$ makes decisions only in the neighborhood of the arm that has the highest empirical mean reward.
We theoretically prove that, for Bernoulli rewards, the upper bound regret of $\texttt{FEF}$-$\texttt{UTS}$ matches the lower asymptotic bound regret of unimodal bandits, thus $\texttt{FEF}$-$\texttt{UTS}$ is an asymptotically optimal algorithm. 
Finally, we use experiments to demonstrate the effectiveness of the proposed algorithm, results show that $\texttt{FEF}$-$\texttt{UTS}$ performs better than extensive state-of-the-art algorithms.
We have opened our code at: \url{https://github.com/jijiaming-bit/FEF-UTS}.
